Genetically Modified Wolf Optimization with Stochastic Gradient Descent for Optimising Deep Neural Networks

When training Convolutional Neural Networks (CNNs) there is a large emphasis on creating efficient optimization algorithms and highly accurate networks. The state-of-the-art method of optimizing the networks is done by using gradient descent algorithms, such as Stochastic Gradient Descent (SGD). However, there are some limitations presented when using gradient descent methods. The major drawback is the lack of exploration, and over-reliance on exploitation. Hence, this research aims to analyze an alternative approach to optimizing neural network (NN) weights, with the use of population-based metaheuristic algorithms. A hybrid between Grey Wolf Optimizer (GWO) and Genetic Algorithms (GA) is explored, in conjunction with SGD; producing a Genetically Modified Wolf optimization algorithm boosted with SGD (GMW-SGD). This algorithm allows for a combination between exploitation and exploration, whilst also tackling the issue of high-dimensionality, affecting the performance of standard metaheuristic algorithms. The proposed algorithm was trained and tested on CIFAR-10 where it performs comparably to the SGD algorithm, reaching high test accuracy, and significantly outperforms standard metaheuristic algorithms.

==> bibliography.tex <==
@article{ZHANG20071026,
title = {A hybrid particle swarm optimization–back-propagation algorithm for feedforward neural network training},
journal = {Applied Mathematics and Computation},
volume = {185},
number = {2},
pages = {1026-1037},
year = {2007},
note = {Special Issue on Intelligent Computing Theory and Methodology},
issn = {0096-3003},
doi = {https://doi.org/10.1016/j.amc.2006.07.025},
url = {https://www.sciencedirect.com/science/article/pii/S0096300306008277},
author = {Jing-Ru Zhang and Jun Zhang and Tat-Ming Lok and Michael R. Lyu},
keywords = {Particle swarm optimization algorithm, Feedforward neural network, BP algorithm, Adaptive particle swarm optimization},
abstract = {The particle swarm optimization algorithm was showed to converge rapidly during the initial stages of a global search, but around global optimum, the search process will become very slow. On the contrary, the gradient descending method can achieve faster convergent speed around global optimum, and at the same time, the convergent accuracy can be higher. So in this paper, a hybrid algorithm combining particle swarm optimization (PSO) algorithm with back-propagation (BP) algorithm, also referred to as PSO–BP algorithm, is proposed to train the weights of feedforward neural network (FNN), the hybrid algorithm can make use of not only strong global searching ability of the PSOA, but also strong local searching ability of the BP algorithm. In this paper, a novel selection strategy of the inertial weight is introduced to the PSO algorithm. In the proposed PSO–BP algorithm, we adopt a heuristic way to give a transition from particle swarm search to gradient descending search. In this paper, we also give three kind of encoding strategy of particles, and give the different problem area in which every encoding strategy is used. The experimental results show that the proposed hybrid PSO–BP algorithm is better than the Adaptive Particle swarm optimization algorithm (APSOA) and BP algorithm in convergent speed and convergent accuracy.}
}

@article{10.2307/24939139,
 ISSN = {00368733, 19467087},
 URL = {http://www.jstor.org/stable/24939139},
 author = {John H. Holland},
 journal = {Scientific American},
 number = {1},
 pages = {66--73},
 publisher = {Scientific American, a division of Nature America, Inc.},
 title = {Genetic Algorithms},
 urldate = {2022-12-05},
 volume = {267},
 year = {1992}
}

@article{albeahdili2015hybrid,
  title={Hybrid algorithm for the optimization of training convolutional neural network},
  author={Albeahdili, Hayder M and Han, Tony and Islam, Naz E},
  journal={Int J Adv Comput Sci Appl},
  volume={1},
  number={6},
  pages={79--85},
  year={2015}
}

@InProceedings{Huang_2017_CVPR,
author = {Huang, Gao and Liu, Zhuang and van der Maaten, Laurens and Weinberger, Kilian Q.},
title = {Densely Connected Convolutional Networks},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
}

@inproceedings{tan2021efficientnetv2,
  title={Efficientnetv2: Smaller models and faster training},
  author={Tan, Mingxing and Le, Quoc},
  booktitle={International Conference on Machine Learning},
  pages={10096--10106},
  year={2021},
  organization={PMLR}
}

@ARTICLE{9877850,
  author={Zhao, Shuai and Zhou, Liguang and Wang, Wenxiao and Cai, Deng and Lam, Tin Lun and Xu, Yangsheng},
  journal={IEEE Transactions on Image Processing}, 
  title={Toward Better Accuracy-Efficiency Trade-Offs: Divide and Co-Training}, 
  year={2022},
  volume={31},
  number={},
  pages={5869-5880},
  doi={10.1109/TIP.2022.3201602}}

  @article{beheshti2013review,
  title={A review of population-based meta-heuristic algorithms},
  author={Beheshti, Zahra and Shamsuddin, Siti Mariyam Hj},
  journal={Int. J. Adv. Soft Comput. Appl},
  volume={5},
  number={1},
  pages={1--35},
  year={2013}
}

@article{bashir2009applying,
  title={Applying wavelets to short-term load forecasting using PSO-based neural networks},
  author={Bashir, ZA and El-Hawary, ME},
  journal={IEEE transactions on power systems},
  volume={24},
  number={1},
  pages={20--27},
  year={2009},
  publisher={IEEE}
}

@article{mirjalili2015effective,
  title={How effective is the Grey Wolf optimizer in training multi-layer perceptrons},
  author={Mirjalili, Seyedali},
  journal={Applied Intelligence},
  volume={43},
  number={1},
  pages={150--161},
  year={2015},
  publisher={Springer}
}

@article{mosavi2016classification,
  title={Classification of sonar data set using neural network trained by gray wolf optimization},
  author={Mosavi, Mohammad Reza and Khishe, Mohammad and Ghamgosar, Abolfazl},
  journal={Neural Network World},
  volume={26},
  number={4},
  pages={393},
  year={2016},
  publisher={Czech Technical University in Prague, Faculty of Transportation Sciences}
}

@INPROCEEDINGS{1202255,
  author={Gudise, V.G. and Venayagamoorthy, G.K.},
  booktitle={Proceedings of the 2003 IEEE Swarm Intelligence Symposium. SIS'03 (Cat. No.03EX706)}, 
  title={Comparison of particle swarm optimization and backpropagation as training algorithms for neural networks}, 
  year={2003},
  volume={},
  number={},
  pages={110-117},
  doi={10.1109/SIS.2003.1202255}}

  @inproceedings{de2021gacnn,
  title={gaCNN: Composing CNNs and GAs to Build an Optimized Hybrid Classification Architecture},
  author={de Lima Mendes, Raphael and da Silva Alves, Alexandre Henrick and de Souza Gomes, Matheus and Bertarini, Pedro Luiz Lima and do Amaral, Laurence Rodrigues},
  booktitle={2021 IEEE Congress on Evolutionary Computation (CEC)},
  pages={79--86},
  year={2021},
  organization={IEEE}
}

@inproceedings{NEURIPS2018_62da8c91,
 author = {Cui, Xiaodong and Zhang, Wei and T\"{u}ske, Zolt\'{a}n and Picheny, Michael},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Evolutionary Stochastic Gradient Descent for Optimization of Deep Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2018/file/62da8c91ce7b10846231921795d6059e-Paper.pdf},
 volume = {31},
 year = {2018}
}

@article{chen2009hybrid,
  title={Hybrid of genetic algorithm and simulated annealing for multiple project scheduling with multiple resource constraints},
  author={Chen, Po-Han and Shahandashti, Seyed Mohsen},
  journal={Automation in Construction},
  volume={18},
  number={4},
  pages={434--443},
  year={2009},
  publisher={Elsevier}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

 @misc{karim_2022, title={Illustrated: 10 CNN Architectures}, url={https://towardsdatascience.com/illustrated-10-cnn-architectures-95d78ace614d}, journal={Medium}, publisher={Towards Data Science}, author={Karim, Raimi}, year={2022}, month={Jan}} 


@inproceedings{kennedy1995particle,
  title={Particle swarm optimization},
  author={Kennedy, James and Eberhart, Russell},
  booktitle={Proceedings of ICNN'95-international conference on neural networks},
  volume={4},
  pages={1942--1948},
  year={1995},
  organization={IEEE}
}

@article{khan2020survey,
  title={A survey of the recent architectures of deep convolutional neural networks},
  author={Khan, Asifullah and Sohail, Anabia and Zahoora, Umme and Qureshi, Aqsa Saeed},
  journal={Artificial intelligence review},
  volume={53},
  number={8},
  pages={5455--5516},
  year={2020},
  publisher={Springer}
}

@article{ZHANG2019109,
title = {Differential mutation and novel social learning particle swarm optimization algorithm},
journal = {Information Sciences},
volume = {480},
pages = {109-129},
year = {2019},
issn = {0020-0255},
doi = {https://doi.org/10.1016/j.ins.2018.12.030},
url = {https://www.sciencedirect.com/science/article/pii/S0020025518309629},
author = {Xinming Zhang and Xia Wang and Qiang Kang and Jinfeng Cheng},
keywords = {Intelligence optimization algorithm, Evolutionary algorithm, Particle swarm optimization, Differential mutation, Social learning},
abstract = {Social Learning Particle Swarm Optimization (SLPSO) is an improved Particle Swarm Optimization (PSO) algorithm, which greatly improves the optimization performance of PSO. However, SLPSO still has some deficiency, such as poor balance between exploration and exploitation and low search efficiency, so that it cannot yet do well in solving many complex optimization problems. Thus, this paper proposes an improved SLPSO algorithm, that is, Differential mutation and novel Social learning PSO (DSPSO). Firstly, in order to balance exploration and exploitation better, a dynamic inertia weight is introduced to replace the random inertia weight of SLPSO, and a single-example learning approach and an example-mean learning one are proposed to replace the imitation component and the social influence component of SLPSO respectively. Secondly, the dimension-based velocity updating equation of SLPSO is divided into two particle-based updating equations with the two approaches, and the two are executed alternately to form a novel social learning PSO (NSLPSO), which enhance the exploitation of SLPSO. Finally, a dynamic differential mutation strategy is used in NSLPSO to update the three best particles to enhance the exploration to obtain DSPSO. Experimental results on the complex functions from CEC2013 reveal that DSPSO outperforms SLPSO and quite a few state-of-the-art and classic PSO variants.}
}

@ARTICLE{6819057,
  author={Cheng, Ran and Jin, Yaochu},
  journal={IEEE Transactions on Cybernetics}, 
  title={A Competitive Swarm Optimizer for Large Scale Optimization}, 
  year={2015},
  volume={45},
  number={2},
  pages={191-204},
  doi={10.1109/TCYB.2014.2322602}}


@article{wolpert1997no,
  title={No free lunch theorems for optimization},
  author={Wolpert, David H and Macready, William G},
  journal={IEEE transactions on evolutionary computation},
  volume={1},
  number={1},
  pages={67--82},
  year={1997},
  publisher={IEEE}
}
@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Toronto, ON, Canada}
}

@incollection{Fong16,
author = {Zhonghuan Tian and Simon Fong},
title = {Survey of Meta-Heuristic Algorithms for Deep Learning Training},
booktitle = {Optimization Algorithms},
publisher = {IntechOpen},
address = {Rijeka},
year = {2016},
editor = {Ozgur Baskan},
chapter = {9},
doi = {10.5772/63785},
url = {https://doi.org/10.5772/63785}
}


@ARTICLE{1275532,  author={Chia-Feng Juang},  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},   title={A hybrid of genetic algorithm and particle swarm optimization for recurrent network design},   year={2004},  volume={34},  number={2},  pages={997-1006},  doi={10.1109/TSMCB.2003.818557}}

@ARTICLE{Rere2016-bs,
  title     = "Metaheuristic algorithms for convolution neural network",
  author    = "Rere, L M Rasdi and Fanany, Mohamad Ivan and Arymurthy, Aniati
               Murni",
  abstract  = "A typical modern optimization technique is usually either
               heuristic or metaheuristic. This technique has managed to solve
               some optimization problems in the research area of science,
               engineering, and industry. However, implementation strategy of
               metaheuristic for accuracy improvement on convolution neural
               networks (CNN), a famous deep learning method, is still rarely
               investigated. Deep learning relates to a type of machine
               learning technique, where its aim is to move closer to the goal
               of artificial intelligence of creating a machine that could
               successfully perform any intellectual tasks that can be carried
               out by a human. In this paper, we propose the implementation
               strategy of three popular metaheuristic approaches, that is,
               simulated annealing, differential evolution, and harmony search,
               to optimize CNN. The performances of these metaheuristic methods
               in optimizing CNN on classifying MNIST and CIFAR dataset were
               evaluated and compared. Furthermore, the proposed methods are
               also compared with the original CNN. Although the proposed
               methods show an increase in the computation time, their accuracy
               has also been improved (up to 7.14 percent).",
  journal   = "Comput. Intell. Neurosci.",
  publisher = "Hindawi Limited",
  volume    =  2016,
  pages     = "1537325",
  month     =  jun,
  year      =  2016,
  language  = "en"
}


@ARTICLE{Amirsadri2018-yo,
  title     = "A Levy flight-based grey wolf optimizer combined with
               back-propagation algorithm for neural network training",
  author    = "Amirsadri, Shima and Mousavirad, Seyed Jalaleddin and
               Ebrahimpour-Komleh, Hossein",
  journal   = "Neural Comput. Appl.",
  publisher = "Springer Science and Business Media LLC",
  volume    =  30,
  number    =  12,
  pages     = "3707--3720",
  month     =  dec,
  year      =  2018,
  language  = "en"
}



@article{MCCALL2005205,
title = {Genetic algorithms for modelling and optimisation},
journal = {Journal of Computational and Applied Mathematics},
volume = {184},
number = {1},
pages = {205-222},
year = {2005},
note = {Special Issue on Mathematics Applied to Immunology},
issn = {0377-0427},
doi = {https://doi.org/10.1016/j.cam.2004.07.034},
url = {https://www.sciencedirect.com/science/article/pii/S0377042705000774},
author = {John McCall},
keywords = {Genetic algorithms, Immunology, Optimisation, Evolution},
abstract = {Genetic algorithms (GAs) are a heuristic search and optimisation technique inspired by natural evolution. They have been successfully applied to a wide range of real-world problems of significant complexity. This paper is intended as an introduction to GAs aimed at immunologists and mathematicians interested in immunology. We describe how to construct a GA and the main strands of GA theory before speculatively identifying possible applications of GAs to the study of immunology. An illustrative example of using a GA for a medical optimal control problem is provided. The paper also includes a brief account of the related area of artificial immune systems.}
}


@INPROCEEDINGS{9185541,
  author={Wang, Bin and Xue, Bing and Zhang, Mengjie},
  booktitle={2020 IEEE Congress on Evolutionary Computation (CEC)}, 
  title={Particle Swarm optimisation for Evolving Deep Neural Networks for Image Classification by Evolving and Stacking Transferable Blocks}, 
  year={2020},
  volume={},
  number={},
  pages={1-8},
  doi={10.1109/CEC48606.2020.9185541}}



@INPROCEEDINGS{488968,  author={Kennedy, J. and Eberhart, R.},  booktitle={Proceedings of ICNN'95 - International Conference on Neural Networks},   title={Particle swarm optimization},   year={1995},  volume={4},  number={},  pages={1942-1948 vol.4},  doi={10.1109/ICNN.1995.488968}}



@article{MIRJALILI201211125,
title = {Training feedforward neural networks using hybrid particle swarm optimization and gravitational search algorithm},
journal = {Applied Mathematics and Computation},
volume = {218},
number = {22},
pages = {11125-11137},
year = {2012},
issn = {0096-3003},
doi = {https://doi.org/10.1016/j.amc.2012.04.069},
url = {https://www.sciencedirect.com/science/article/pii/S0096300312004857},
author = {SeyedAli Mirjalili and Siti Zaiton {Mohd Hashim} and Hossein {Moradian Sardroudi}},
keywords = {FNN, Neural network, Learning neural network, Gravitational search algorithm, Particle swarm optimization, PSO, Evolutionary algorithm, Multilayer perceptron},
abstract = {The Gravitational Search Algorithm (GSA) is a novel heuristic optimization method based on the law of gravity and mass interactions. It has been proven that this algorithm has good ability to search for the global optimum, but it suffers from slow searching speed in the last iterations. This work proposes a hybrid of Particle Swarm Optimization (PSO) and GSA to resolve the aforementioned problem. In this paper, GSA and PSOGSA are employed as new training methods for Feedforward Neural Networks (FNNs) in order to investigate the efficiencies of these algorithms in reducing the problems of trapping in local minima and the slow convergence rate of current evolutionary learning algorithms. The results are compared with a standard PSO-based learning algorithm for FNNs. The resulting accuracy of FNNs trained with PSO, GSA, and PSOGSA is also investigated. The experimental results show that PSOGSA outperforms both PSO and GSA for training FNNs in terms of converging speed and avoiding local minima. It is also proven that an FNN trained with PSOGSA has better accuracy than one trained with GSA.}
}


@article{CHENG201543,
title = {A social learning particle swarm optimization algorithm for scalable optimization},
journal = {Information Sciences},
volume = {291},
pages = {43-60},
year = {2015},
issn = {0020-0255},
doi = {https://doi.org/10.1016/j.ins.2014.08.039},
url = {https://www.sciencedirect.com/science/article/pii/S0020025514008366},
author = {Ran Cheng and Yaochu Jin},
keywords = {Social learning, Particle swarm optimization, Large-scale optimization, Computational efficiency, Scalability},
abstract = {Social learning plays an important role in behavior learning among social animals. In contrast to individual (asocial) learning, social learning has the advantage of allowing individuals to learn behaviors from others without incurring the costs of individual trials-and-errors. This paper introduces social learning mechanisms into particle swarm optimization (PSO) to develop a social learning PSO (SL-PSO). Unlike classical PSO variants where the particles are updated based on historical information, including the best solution found by the whole swarm (global best) and the best solution found by each particle (personal best), each particle in the proposed SL-PSO learns from any better particles (termed demonstrators) in the current swarm. In addition, to ease the burden of parameter settings, the proposed SL-PSO adopts a dimension-dependent parameter control method. The proposed SL-PSO is first compared with five representative PSO variants on 40 low-dimensional test functions, including shifted and rotated test functions. The scalability of the proposed SL-PSO is further tested by comparing it with five state-of-the-art algorithms for large-scale optimization on seven high-dimensional (100-D, 500-D, and 1000-D) benchmark functions. Our comparative results show that SL-PSO performs well on low-dimensional problems and is promising for solving large-scale problems as well.}
}

@ARTICLE{Barrera2016-kt,
  title     = "Limiting the velocity in the particle swarm optimization
               algorithm",
  author    = "Barrera, Julio and {\'A}lvarez Bajo, Osiris and Flores, Juan J
               and Coello Coello, Carlos A",
  journal   = "Comput. sist.",
  publisher = "Instituto Politecnico Nacional/Centro de Investigacion en
               Computacion",
  volume    =  20,
  number    =  4,
  month     =  dec,
  year      =  2016
}


@book{10.5555/1557464,
author = {Engelbrecht, Andries P.},
title = {Computational Intelligence: An Introduction},
year = {2007},
isbn = {0470035617},
publisher = {Wiley Publishing},
edition = {2nd},
abstract = {Computational Intelligence: An Introduction, Second Edition offers an in-depth exploration into the adaptive mechanisms that enable intelligent behaviour in complex and changing environments. The main focus of this text is centred on the computational modelling of biological and natural intelligent systems, encompassing swarm intelligence, fuzzy systems, artificial neutral networks, artificial immune systems and evolutionary computation. Engelbrecht provides readers with a wide knowledge of Computational Intelligence (CI) paradigms and algorithms; inviting readers to implement and problem solve real-world, complex problems within the CI development framework. This implementation framework will enable readers to tackle new problems without any difficulty through a single Java class as part of the CI library. Key features of this second edition include: A tutorial, hands-on based presentation of the material. State-of-the-art coverage of the most recent developments in computational intelligence with more elaborate discussions on intelligence and artificial intelligence (AI). New discussion of Darwinian evolution versus Lamarckian evolution, also including swarm robotics, hybrid systems and artificial immune systems. A section on how to perform empirical studies; topics including statistical analysis of stochastic algorithms, and an open source library of CI algorithms. Tables, illustrations, graphs, examples, assignments, Java code implementing the algorithms, and a complete CI implementation and experimental framework. Computational Intelligence: An Introduction, Second Edition is essential reading for third and fourth year undergraduate and postgraduate students studying CI. The first edition has been prescribed by a number of overseas universities and is thus a valuable teaching tool. In addition, it will also be a useful resource for researchers in Computational Intelligence and Artificial Intelligence, as well as engineers, statisticians, operational researchers, and bioinformaticians with an interest in applying AI or CI to solve problems in their domains. Check out http://www.ci.cs.up.ac.za for examples, assignments and Java code implementing the algorithms.}
}


@ARTICLE{Chong2021-pn,
  title     = "Advances of metaheuristic algorithms in training neural networks
               for industrial applications",
  author    = "Chong, Hue Yee and Yap, Hwa Jen and Tan, Shing Chiang and Yap,
               Keem Siah and Wong, Shen Yuong",
  journal   = "Soft Comput.",
  publisher = "Springer Science and Business Media LLC",
  volume    =  25,
  number    =  16,
  pages     = "11209--11233",
  month     =  aug,
  year      =  2021,
  language  = "en"
}


@article{MIRJALILI201446,
title = {Grey Wolf Optimizer},
journal = {Advances in Engineering Software},
volume = {69},
pages = {46-61},
year = {2014},
issn = {0965-9978},
doi = {https://doi.org/10.1016/j.advengsoft.2013.12.007},
url = {https://www.sciencedirect.com/science/article/pii/S0965997813001853},
author = {Seyedali Mirjalili and Seyed Mohammad Mirjalili and Andrew Lewis},
keywords = {Optimization, Optimization techniques, Heuristic algorithm, Metaheuristics, Constrained optimization, GWO},
abstract = {This work proposes a new meta-heuristic called Grey Wolf Optimizer (GWO) inspired by grey wolves (Canis lupus). The GWO algorithm mimics the leadership hierarchy and hunting mechanism of grey wolves in nature. Four types of grey wolves such as alpha, beta, delta, and omega are employed for simulating the leadership hierarchy. In addition, the three main steps of hunting, searching for prey, encircling prey, and attacking prey, are implemented. The algorithm is then benchmarked on 29 well-known test functions, and the results are verified by a comparative study with Particle Swarm Optimization (PSO), Gravitational Search Algorithm (GSA), Differential Evolution (DE), Evolutionary Programming (EP), and Evolution Strategy (ES). The results show that the GWO algorithm is able to provide very competitive results compared to these well-known meta-heuristics. The paper also considers solving three classical engineering design problems (tension/compression spring, welded beam, and pressure vessel designs) and presents a real application of the proposed method in the field of optical engineering. The results of the classical engineering design problems and real application prove that the proposed algorithm is applicable to challenging problems with unknown search spaces.}
}

@article{NOEL2012353,
title = {A new gradient based particle swarm optimization algorithm for accurate computation of global minimum},
journal = {Applied Soft Computing},
volume = {12},
number = {1},
pages = {353-359},
year = {2012},
issn = {1568-4946},
doi = {https://doi.org/10.1016/j.asoc.2011.08.037},
url = {https://www.sciencedirect.com/science/article/pii/S1568494611003206},
author = {Mathew M. Noel},
keywords = {Particle swarm optimization (PSO), Gradient descent, Global optimization techniques, Stochastic optimization},
abstract = {Stochastic optimization algorithms like genetic algorithms (GAs) and particle swarm optimization (PSO) algorithms perform global optimization but waste computational effort by doing a random search. On the other hand deterministic algorithms like gradient descent converge rapidly but may get stuck in local minima of multimodal functions. Thus, an approach that combines the strengths of stochastic and deterministic optimization schemes but avoids their weaknesses is of interest. This paper presents a new hybrid optimization algorithm that combines the PSO algorithm and gradient-based local search algorithms to achieve faster convergence and better accuracy of final solution without getting trapped in local minima. In the new gradient-based PSO algorithm, referred to as the GPSO algorithm, the PSO algorithm is used for global exploration and a gradient based scheme is used for accurate local exploration. The global minimum is located by a process of finding progressively better local minima. The GPSO algorithm avoids the use of inertial weights and constriction coefficients which can cause the PSO algorithm to converge to a local minimum if improperly chosen. The De Jong test suite of benchmark optimization problems was used to test the new algorithm and facilitate comparison with the classical PSO algorithm. The GPSO algorithm is compared to four different refinements of the PSO algorithm from the literature and shown to converge faster to a significantly more accurate final solution for a variety of benchmark test functions.}
}

@article{robbins1951stochastic,
  title={A stochastic approximation method},
  author={Robbins, Herbert and Monro, Sutton},
  journal={The annals of mathematical statistics},
  pages={400--407},
  year={1951},
  publisher={JSTOR}
}

@ARTICLE{8329968,  author={Daniel, Ebenezer},  journal={IEEE Sensors Journal},   title={Optimum Wavelet-Based Homomorphic Medical Image Fusion Using Hybrid Genetic–Grey Wolf Optimization Algorithm},   year={2018},  volume={18},  number={16},  pages={6804-6811},  doi={10.1109/JSEN.2018.2822712}}

@article{XUE2022453,
title = {An ensemble of differential evolution and Adam for training feed-forward neural networks},
journal = {Information Sciences},
volume = {608},
pages = {453-471},
year = {2022},
issn = {0020-0255},
doi = {https://doi.org/10.1016/j.ins.2022.06.036},
url = {https://www.sciencedirect.com/science/article/pii/S0020025522006260},
author = {Yu Xue and Yiling Tong and Ferrante Neri},
keywords = {Feed-forward neural networks, Multi-populations, Ensemble algorithms, Differential algorithms, Gradient-based algorithms},
abstract = {Adam is an adaptive gradient descent approach that is commonly used in back-propagation (BP) algorithms for training feed-forward neural networks (FFNNs). However, it has the defect that it may easily fall into local optima. To solve this problem, some metaheuristic approaches have been proposed to train FFNNs. While these approaches have stronger global search capabilities enabling them to more readily escape from local optima, their convergence performance is not as good as that of Adam. The proposed algorithm is an ensemble of differential evolution and Adam (EDEAdam), which integrates a modern version of the differential evolution algorithm with Adam, using two different sub-algorithms to evolve two sub-populations in parallel and thereby achieving good results in both global and local search. Compared with traditional algorithms, the integration of the two algorithms endows EDEAdam with powerful capabilities to handle different classification problems. Experimental results prove that EDEAdam not only exhibits improved global and local search capabilities, but also achieves a fast convergence speed.}
}

@ARTICLE{996017,
  author={Deb, K. and Pratap, A. and Agarwal, S. and Meyarivan, T.},
  journal={IEEE Transactions on Evolutionary Computation}, 
  title={A fast and elitist multiobjective genetic algorithm: NSGA-II}, 
  year={2002},
  volume={6},
  number={2},
  pages={182-197},
  doi={10.1109/4235.996017}}

